An efficient null space inexact Newton method for hydraulic simulation of water distribution networks

Null space Newton algorithms are efficient in solving the nonlinear equations arising in hydraulic analysis of water distribution networks. In this article, we propose and evaluate an inexact Newton method that relies on partial updates of the network pipes' frictional headloss computations to solve the linear systems more efficiently and with numerical reliability. The update set parameters are studied to propose appropriate values. Different null space basis generation schemes are analysed to choose methods for sparse and well-conditioned null space bases resulting in a smaller update set. The Newton steps are computed in the null space by solving sparse, symmetric positive definite systems with sparse Cholesky factorizations. By using the constant structure of the null space system matrices, a single symbolic factorization in the Cholesky decomposition is used multiple times, reducing the computational cost of linear solves. The algorithms and analyses are validated using medium to large-scale water network models.

==> CPUstack_2.tex <==
\pgfplotstableread{ % Read the data into a table macro
Label   First   Second  Third   Fourth Csum
%{Schur-Alg}    15.6600    5.1560    5.2000    9.9640     35.9800	
NSM1    3.7180    4.4200    4.8600    3.1020      16.1000
NSM2    3.6960    2.5400    3.4800    4.7040   	  14.4200
NSM3    1.5220    2.6140    3.5200    3.9640	  11.6200
}\datatable

\begin{tikzpicture}
\begin{axis}[
    xbar stacked,
    xlabel near ticks,
    xlabel={CPU time (ms)},
    xlabel style={at={(xticklabel cs:0.5)},name=myxlabel},
    legend style={
        legend columns=3,%number of legends per line
        at={(myxlabel.south)},%{(xticklabel cs:0.4)},
        anchor=north,
        draw=none
    },
%     title style={at={(xticklabel cs:0.9), ( yticklabel cs:-.2)}},title={CPU time (ms)},
    ytick=data,
    axis y line*=left,
    axis x line*=bottom,
    tick label style={font=\footnotesize},
    legend style={font=\footnotesize},    
    label style={font=\footnotesize},
    xtick={0,2,4,6,8,10,12,14,16},
    width=0.5\textwidth,
    bar width=6mm,
    yticklabel style={text width=8mm},%, align=right},
    yticklabels from table={\datatable}{Label},
    xmin=0,
%     xmax=100.1,
    y=8mm,
    enlarge y limits=0.5,
    point meta=explicit,
%%%% Activate bar numbers here to
    every node near coord/.style={
      check for zero/.code={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{\pgfplotspointmeta}
        \pgfmathfloatifflags{\pgfmathresult}{-}{
           \pgfkeys{/tikz/coordinate}
        }{}
        \pgfkeys{/pgf/fpu=false}
      }, check for zero, xshift=3, font=\bfseries},
    nodes near coords={\pgfmathprintnumber[fixed zerofill,precision=1]{\pgfplotspointmeta}},
%%%%% end bar numbers here
    nodes near coords align=left
]

%%%%Plot without numbers on bars
% \addplot [draw=black, pattern color = red, pattern = horizontal lines,area legend] table [x=First, y expr=\coordindex] {\datatable}; 
% \addplot [draw=black, pattern color = red!50!green, pattern = north west lines,area legend]table [x=Second, y expr=\coordindex] {\datatable};
% \addplot [draw=black, pattern color = cyan, pattern = vertical lines, area legend] table [x=Third, y expr=\coordindex] {\datatable};
% \addplot [draw=black,fill=blue!60!yellow, area legend] table [x=Fourth, y expr=\coordindex] {\datatable};
%%Plot with numbers on bars
\addplot [draw=black, pattern color = red, pattern = north east lines,area legend] table [x=First, y expr=\coordindex, meta expr=\thisrow{First}] {\datatable}; 
\addplot [draw=black, pattern color = red!50!green, pattern = horizontal lines,area legend]table [x=Second, y expr=\coordindex,meta expr=\thisrow{Second}] {\datatable};
\addplot [draw=black, pattern color = cyan, pattern = dots, area legend] table [x=Third, y expr=\coordindex,meta expr=\thisrow{Third}] {\datatable};
\addplot [draw=black,fill=lightgray, area legend] table [x=Fourth, y expr=\coordindex,meta expr=\thisrow{Fourth}] {\datatable};
%%%%%Plot with percentages
% \addplot [draw=black, pattern color = red, pattern = horizontal lines,area legend] table [x=First, y expr=\coordindex, meta expr=(\thisrow{First}*100)/\thisrow{Csum}] {\datatable}; 
% \addplot [draw=black, pattern color = red!50!green, pattern = north west lines,area legend]table [x=Second, y expr=\coordindex,meta expr=\thisrow{Second}*100/\thisrow{Csum}] {\datatable};
% \addplot [draw=black, pattern color = cyan, pattern = vertical lines, area legend] table [x=Third, y expr=\coordindex,meta expr=\thisrow{Third}*100/\thisrow{Csum}] {\datatable};
% \addplot [draw=black,fill=blue!60!yellow, area legend] table [x=Fourth, y expr=\coordindex,meta expr=\thisrow{Fourth}*100/\thisrow{Csum}] {\datatable};
%%%
\legend{Linear Solver,Head Loss,Matrix-Matrix Muls,Others};
\end{axis}
\end{tikzpicture}
